Configuration Space Methods and Time Ordering for Scalar Propagators in (Anti and) de Sitter Spacetimes

In this master thesis a configuration space method presented by C. Dullemond and E. van Beveren for computing all propagators of a scalar field (Wightman, Hadamard and Schwinger functions,retarded, advanced and Feynman propagator) is reviewed for four-dimensional Minkowski and Anti de Sitter spacetime AdS_4. This method is then applied for AdS_d as well as de Sitter spacetime dS_d of arbitrary dimension d, obtaining results in agreement with the literature. The advantages of the method are that it needs neither mode summation nor analytic continuation from euclidean time, while delivering the propagators above including (i-epsilon)-prescription, plus as a nice bonus the conformal dimension of a corresponding CFT field. General properties of the considered spacetimes (namely various coordinate systems and their metrics, chordal distances, relations between conformal dimensions \Delta and the mass m of the scalar field, geodesics and the invariance of time ordering) are also examined and compiled from various sources, providing an overview of geometrical properties of AdS and dS spacetimes.

==> dvb_ds_delnorm_xy.tex <==
%%
In order to construct the Feynman propagator fulfilling the inhomogeneous
Klein-Gordon equation (\ref{eq:dvb_ds29_5}), we again need to show
that applying the Klein-Gordon operator to our candidate functions
yields the desired delta source.
\\
According to (\ref{eq:dvb_ds29}) we therefor shall examine
$\bigl( \del_{\tau_x} \phi_\Delta^\pm \bigr)_{\!\tau_x=\tau_y}$ \!\!
in order to show that it delivers a delta function
for the spatial variables $\vec{\phii}_{x,y}$
of the spacetime points $x$ and $y$.
Likewise to the AdS case we plan to identify
$\phi_\Delta^\pm$ with $G^{\mp}_\Delta$. \\
%%
Starting from equation (\ref{eq:dvb_ds_57_5})
and employing (\ref{eq:hypergeo04_5}) we get 
%%
\begin{align}
	\label{eq:dvb_ds57_7}
	\phi^\pm_{\! \Delta}{\ssty \! ( \! \lambda_\pm \!)} \, 
	= \, \bigl(1\!-\! \lambda_\pm \bigr)^{1-d/2}
	F \bigl( c\!-\!a, \, c\!-\!b, \, c, \, \lambda_\pm \bigr)
\end{align}
%%
Next we put to work the chain rule of differentiation
$(\del_{\tau_x} \phi_\Delta^\pm) = (\del_{\tau_x} \lambda_\pm)
(\del_{\lambda_\pm} \phi_\Delta^\pm)$
wherein for the last factor we can make use of equation (\ref{eq:hypergeo04}).
%%
\begin{align}
	\label{eq:dvb_ds58}
	\Bigl( \del_{\tau_x}
	\phi^\pm_\Delta {\ssty \! ( \! \lambda_{\! \pm} \!)} \! \Bigr)_{\! %%@
\tau_x=\tau_y} \!\!\!
	& = \, \bigl( \del_{\tau_x} \lambda_\pm \bigr)_{\! \tau_x=\tau_y}
			\Bigl[
			({\ssty \frac{d}{2}}\!-\!1) (1\!-\! \lambda_\pm )^{-\frac{d}{2}}
			F { \ssty( c\!-\!a, \, c\!-\!b, \, c, \, \lambda_\pm)} \\
			& \qquad \qquad \qquad \quad \;\;
			+ {\ssty \frac{(c-a)(c-b)}{c}} (1\!-\! \lambda_\pm )^{1-\frac{d}{2}}
			F {\ssty (c-a+1,c-b+1,c+1, \lambda_\pm)}
			\Bigr]_{\! \tau_x=\tau_y} \notag
\end{align}
%%
From equation (\ref{eq:dvb_ds_57_2}) we can read off
%%
\begin{align}
	\label{eq:dvb_ds60}
	\Bigl( \del_{\tau_x} \lambda_\pm \! \Bigr)_{\! \tau_x=\tau_y} \!
	& = \,\epsilon \Bigl( \pm \, {\ssty \frac{i}{4R\ds}}
			- {\ssty \frac{1}{4\epsilon} \, }
			(1 \! - \vec{\xi}_x \vec{\xi}_y) \sinh 2 \tau_x \Bigr)
			\\
	\Bigl( \lambda_\pm \! \Bigr)_{\! \tau_x=\tau_y} \!
	& = \, {\ssty \frac{1}{2}} - {\ssty \frac{1}{4}}
	\Bigl[  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh 2\tau_x
			   - (1 \! + \! \vec{\xi}_x \vec{\xi}_y)
			   + {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \Bigr] 
\end{align}
%%
which for the reference point $\! \vec{\phii}_y \! = \! 0$
(with $\tau_y$ not necessarily zero)
reduces to the simpler expression
%%
\begin{align}
	\Bigl( \lambda_\pm \! \Bigr)_{\! \tau_x=\tau_y} \!
	& = \, {\ssty \frac{1}{2}} - {\ssty \frac{1}{4}}
	\Bigl[  (1 \! - \! \cos \phii^1_x) \cosh 2\tau_x
				- (1 \! + \! \cos \phii^1_x)
				+ {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \Bigr]
		\notag \\ 
	& = \, 1 - {\ssty \frac{1}{2}} (1 \! - \! \cos \phii^1_x) \cosh^2 \! \tau_x 
				- {\ssty \frac{\epsilon^2}{8R^2\ds} \,}
\end{align}
%%
We already found that $(1 \! - \! \lambda_\pm)=\epsilon^2$
iff $(\vec{\xi}_x \! =\vec{\xi}_y)$ i.e. iff $(\vec{\phii}_x \! =\vec{\phii}_y)$.
%%
This means that for all $\vec{\phii}_x \neq \vec{\phii}_y$
we can let $\epsilon$ run to zero so that $( \del_{\tau_x} \! \phi^\pm_\Delta
{\ssty \! ( \! \lambda_{\! \pm} \!)} )_{\tau_x=\tau_y}$ vanishes in this case.
\\
In order to determine suitable normalization constants we need to integrate
$(\del_{\tau_x} \phi_\Delta^\pm )_{\tau_x=\tau_y}$ over S$^{d-1}$.
%%
Doing this, we find that the second summand in equation (\ref{eq:dvb_ds58})
yields a contribution proportional to $\epsilon^2$ 
which therefore vanishes in the limit of small $\epsilon$.
\\
When turning to the first summand,
we first compute the S$^{d- \!1}$-integral
over $\epsilon\, \sqrt{g} \, (1\! / \!-\!\lambda_\pm)^{-d/2}_{\tau_x=\tau_y}$
for the case of our reference point $\vec{\phii}_y \! = \! 0$
and find using integral (\ref{eq:delta155}):
%%
\begin{align}
	\int \limits_{S^{d-1}} \!\!\!\! d^{d-\!1} \phii \,
	\frac{\epsilon \, \sqrt{g}}
			{\bigl( 1 \! - \! \lambda_\pm \bigr)^{\! \frac{d}{2}}_{\tau_x=\tau_y}} \,
	& = \, \frac{2 \pi^{\frac{d\!-\!1}{2}}}{\Gamma({\ssty \frac{d-1}{2}})}
			\, R\ds^d \! \int \limits_0^\pi \!\! d\phii_x^1 
			\, \frac{\, \epsilon \, \cosh^{d-1} \! \tau_x \, \sin^{d-2} \! \phii_x^1}
			{\Bigl[{\ssty \frac{1}{2}} (1 \! - \! \cos \phii_x^1) \cosh^2 \! \tau_x 
			+ {\ssty \frac{\epsilon^2}{8R^2\ds}} \, \Bigr]^{\! \frac{d}{2}}}
	\notag \\
	%%
	& = \, \frac{2 \pi^{\frac{d\!-\!1}{2}}}{\Gamma({\ssty \frac{d-1}{2}})}
			\, R\ds^d \!\!\! \int \limits_0^{\mu \ll 1} \!\!\!\! d\phii_x^1
			\, \frac{\, \epsilon \, \cosh^{d-1} \! \tau_x \, \sin^{d-2} \! \phii_x^1}
			{\Bigl[{\ssty \frac{1}{2}} (1 \! - \! \cos \phii_x^1) \cosh^2 \! \tau_x \!
			+ {\ssty \frac{\epsilon^2}{8R^2\ds}} \, \Bigr]^{\! \frac{d}{2}}}
	\notag \\
	& \qquad \quad
		 	+ \,  \frac{2 \pi^{\frac{d\!-\!1}{2}}}{\Gamma({\ssty \frac{d-1}{2}})}
			\, R\ds^d \!\!\! 
			\ub{ \int \limits_{\mu \ll 1}^\pi \!\!\!\! d\phii_x^1
			\, \frac{\, \epsilon \, \cosh^{d-1} \! \tau_x \, \sin^{d-2} \! \phii_x^1}
			{\Bigl[{\ssty \frac{1}{2}} (1 \! - \! \cos \phii_x^1) \cosh^2 \! \tau_x \! 
			+ {\ssty \frac{\epsilon^2}{8R^2\ds}} \, \Bigr]^{\! \frac{d}{2}}}
			}_{\limepszero \text{exists:} \,  \longrightarrow \, 0}
	\notag \\
	%%
	& \!\! \overset{\epsilon \rightarrow 0}{=} 
			\, \frac{2 \pi^{\frac{d\!-\!1}{2}}}{\Gamma({\ssty \frac{d-1}{2}})}
			\, R\ds^{d+1} 2^{d+\frac{1}{2}} \!\!
			\int \limits_0^\infty \!\! d \phii^1_x \, \frac{\phii_x^{1^{d-2}}}
			{\bigl( \phii_x^{1^2} \!\! + 1  \bigr)^{\! \frac{d}{2}}}
	\notag \\
	& = \; \frac{\, R\ds^{d-1} \, \pi^{\frac{d}{2}}}{\Gamma({\ssty \frac{d}{2}})}
				\; 2^{d+\frac{1}{2}}
	\\
\end{align}
%%
In the first line of the integration above we already used $\sqrt{g}$.
%%
\begin{align}	
	\Longrightarrow \quad \limepszero 
		\frac{\, \epsilon \, \sqrt{g} }
		{(1 \! - \! \lambda_\pm)_{\tau_x=\tau_y}^{\frac{d}{2}}} \;
	& = \; \frac{\, R\ds^{d-1} \, \pi^{\frac{d}{2}}}{\Gamma({\ssty \frac{d}{2}})}
			\; 2^{d+\frac{1}{2}} \,
			\delta^{(\!d\!-\!1\!)}{\ssty (\vec{\phii}_x-\vec{\phii}_y)}
\end{align}
%%
Looking at (\ref{eq:dvb_ds60}) we see
that for $(\vec{\phii}_y = \vec{\phii}_x)$
i.e. $(\vec{\xi}_y = \vec{\xi}_x)$ we have
$\bigl( \del_{\tau_x} \lambda_\pm \! \bigr)_{\! \tau_x=\tau_y} \!
			= \, \pm i {\ssty \frac{\epsilon}{4R\ds}}$.
%%
Therefore using (\ref{eq:hypergeo03_5})
we arrive at the desired spatial delta function:
%%
\begin{align}
	 \sqrt{g} \; \limepszero	\Bigl( \del_{\tau_x} 
			\phi^\pm_\Delta{\ssty \! ( \! \lambda_{\! \pm} \!)} \Bigr)
			_{\! \tau_x=\tau_y}
	& = \; \pm i \, \ub{ \frac{\, (4\pi)^{\! \frac{d}{2}} R\ds^{d-2}\;
		\Gamma({\ssty \frac{d}{2})}}
		{\, \Gamma({\ssty \Delta_+}) \, \Gamma({\ssty \Delta_-})}
		\frac{1}{\sqrt{8}}}_{\beta_\phi} \,		
		\delta^{(\!d\!-\!1\!)} {\ssty (\vec{\phii}_x-\vec{\phii}_y)}
\end{align}
%%
With this relation fixed we can now identify
(up to $\sqrt{g}$ which is already included)
according to (\ref{eq:dvb_gen_ident}):
%%
\begin{align}
	\label{eq:dvb_ds67}
	G_{\! \Delta}^\pm {\ssty (\!x\!,y\!)} \,
	& = \, \frac{1}{\, 2 \beta_\phi \beta_G} \;\;
			\limepszero \, \phi^\mp_\Delta{\ssty \! ( \! \lambda_{\! \mp})}
	\\
	& = \, \ub{\frac{\, \Gamma({\ssty \Delta_+}) \, \Gamma({\ssty \Delta_-})}
					{\, (4\pi)^{\! \frac{d}{2}} R\ds^{d-4}\; \Gamma({\ssty \frac{d}{2})}}
			\frac{\sqrt{8}}{2}}_{1/(2\beta)} \;
			\limepszero \, \phi^\mp_\Delta{\ssty \! ( \! \lambda_{\! \mp})}
	\notag
\end{align}
%%
and construct the other propagators according to
(\ref{eq:dvb_ads03}-\ref{eq:dvb_ads08}).
%%
Evaluating equation (\ref{eq:dvb_ds29})
we find that the Feynman propagator fulfills
the inhomogeneous Klein-Gordon equation (\ref{eq:dvb_ds29_5})
with one delta source on its right hand side:
%%
\begin{align*}
	\left( \sigma \Box _x \!\! + m^{ 2} \right)
	G \! _F^{\,\Delta} {\ssty(\!x\!,y\!)} \; & = \;\,
	\frac{-i}{\sqrt{g}} \;
	\delta^{\! (\!d\!)} {\ssty \! (\!x-y\!)}
	\notag \\
	\left(\Box _x \!\! + \sigma m^{ 2} \right)
	G \! _F^{\,\Delta} {\ssty(\!x\!,y\!)} \; 
	& = \;\frac{ -i \sigma }{\sqrt{g}} \;
	 \delta^{\! (\!d\!)} {\ssty \! (\!x-y\!)}
\end{align*}
%%
The normalization constant is:
%%
\begin{align}
	\beta & = \, \frac{\, (4\pi)^{\! \frac{d}{2}} R\ds^{d-4}\;
					 \Gamma({\ssty \frac{d}{2})}}
					 {\, \Gamma({\ssty \Delta_+}) \, \Gamma({\ssty \Delta_-})}
					\frac{1}{\sqrt{8}}
\end{align}
%%
Again we do not want the $\Gamma{\ssty (\ldots)}$ functions
in our normalization constant to run to infinity.
%%
This requirement is fulfilled for all $m^2R^2\ds > 0$.
%%
In this case $\Delta_\pm$ are either positive or complex
and thus the Gamma functions remain finite
(see discussion above equation \ref{eq:dvb_ds40_5}).
%%


==> dvb_ds_infshift_xy.tex <==
%%
In order to remove this we apply again shifts in the complex $X^0$-plane
%%
\begin{align}
	X^0 \; & \rightarrow \; X^0 \pm \, i {\ssty \frac{\epsilon}{2}}  \\
	Y^0 \; & \rightarrow \; Y^0 \mp \, i {\ssty \frac{\epsilon}{2}}  \notag
\end{align}
%%
which do not change the d'Alembertian.
%%
Next we define:
%%
\begin{align}
	\lambda_\pm \, & = \,\; \frac{1}{2} + \, \frac{X_\pm Y_\pm}{2R\ds^2} \quad
		= \, \frac{\,1\!-\!\sigma}{2} - \frac{u_\pm}{\,4 R\ds^2}
		\qquad \qquad {\ssty u_\pm = (X_{\!\pm} \!-\!Y_{\!\pm})^2} \\
	\ovl{\lambda}_\pm \, & = \,\; \frac{1}{2} - \, \frac{X_\pm Y_\pm}{2R\ds^2}
		\quad = \, \frac{\,1\!+\!\sigma}{2} + \frac{u_\pm}{\,4 R\ds^2}
\end{align}
%%
This definition of $\lambda_\pm$ yields
%%
\begin{align}
	\label{eq:dvb_ds_57_2}
	\lambda_\pm = \, \frac{1}{2} + \frac{\sigma}{4}
		\biggl[  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! + \! \tau_y)
			  & - (1 \! + \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! - \! \tau_y)
			  \quad \\
		& \quad
		\mp i {\ssty \frac{\epsilon}{R^2\ds}} \bigl( X^0 \! - \! Y^0 \bigr) 
		+ {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \biggr]
		\notag
\end{align}
%%
so that we have again 
$\lambda_\pm {\ssty (\!x\!,y\!)}
= \lambda^*_\mp {\ssty (\!x\!,y\!)}
= \lambda_\mp {\ssty (\!y\!,x\!)}$.
%%
$\lambda$ is SO$\ssty (1,d)$ invariant
and sign$(X^0 \! - \! Y^0)$ is invariant under orthochronous SO$\ssty (1,d)$
just as in Minkowski spacetime.
%%
Moreover in the limit of small $\epsilon$ we can replace
$\epsilon (X^0 \! - \! Y^0)$ by $\epsilon R\ds (\tau_x \! - \tau_y)$
(see subsection \ref{sec:ds_timord_ttau}).  
\\
While the $i\epsilon$ term is present, the point 1 is always evaded.
%%
We observe that the $i\epsilon$ term vanishes only
iff $X^0 = Y^0$ i.e. iff $\tau_x\!\!=\!\tau_y$.
%%
In this case we have
%%
\begin{align*}
	\lambda_{\pm (\tau_x=\tau_y\!)} = \, \frac{1}{2} + \frac{\sigma}{4}
	\biggl[  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh 2\tau_x
			   - (1 \! + \! \vec{\xi}_x \vec{\xi}_y)
			   + {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \biggr]
	\\
	\ovl{\lambda}_{\pm (\tau_x=\tau_y\!)} = \, \frac{1}{2} - \frac{\sigma}{4}
	\biggl[  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh 2\tau_x
			   - (1 \! + \! \vec{\xi}_x \vec{\xi}_y)
			   + {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \biggr]
\end{align*}
%%
and thus
%%
\begin{align}
	\label{eq:dvb_ds57_45}
	\lambda^{\sigma=-1}_{\pm (\tau_x=\tau_y\!)} \!
	= \; \ovl{\lambda}^{\sigma=+1}_{\pm (\tau_x=\tau_y\!)} \,
	\leq \, 1 - {\ssty \frac{\epsilon^2}{8R^2\ds}}
	\\
	\lambda^{\sigma=+1}_{\pm (\tau_x=\tau_y\!)}
	= \; \ovl{\lambda}^{\sigma=-1}_{\pm (\tau_x=\tau_y\!)} \,
	\geq \, 0 + {\ssty \frac{\epsilon^2}{8R^2\ds}}
\end{align}
%%
We see that in the upper line
$\lambda_\pm$ is always separated from 1 by $\epsilon^2$ 
while in the lower line $\lambda_\pm$ crosses 1.
%%
Thereby it is clear that $\lambda$ is the right quantity for $\sigma=-1$
and $\ovl{\lambda}$ is the right one for $\sigma=+1$.
%%
This assignment is confirmed by the observation
that for vanishing chordal distance $u=0$
we obtain $\lambda^{\sigma=-1} \! =\ovl{\lambda}^{\sigma=+1} \! =1$
which lets the candidate functions become singular
exactly on the lightcone of the coincident point  
$(X=Y)$ in embedding space i.e. $(x=y)$ in dS.
%%
The opposite assignment would let them become singular
on the lightcone of the antipode point $x=\snake{y}$.
\\
The singularity of our assignment is of delta function type
and realized in the limit of small $\epsilon$
while the singularity of the opposite assignment
is not of delta type since the point 1 is directly crossed.
%%
Moreover in (\ref{eq:dvb_ds57_7}) we can see
that for $d>4$ the singularity of order $(1-{\ssty \frac{d}{2}})<1$.
%%
Hence $\lambda_\pm=1$ is no residual
and does not contribute in integrals like (\ref{eq:solvinhom_integral}).
\\
Therefore we will only consider the case (\ref{eq:dvb_ds57_45})
and from here on simplify our notation to
$\lambda_\pm=\lambda^{\sigma=-1}_\pm=\ovl{\lambda}^{\sigma=+1}_\pm$.
\\
We remark that $\lambda_{\pm (\tau_x=\tau_y\!)} =1-\epsilon^2$
iff $\vec{\xi}_x = \vec{\xi}_y$.
%%
After all we have found a well defined candidate function:
%%
\beq
	\label{eq:dvb_ds_57_5}
	\phi^\pm_{\! \Delta}{\scriptstyle \! ( \! \lambda_\pm \!)} \, 
	= \, F (a,b,c, \lambda_\pm) \,
	= \, F \Bigl(\Delta_+, \Delta_-,\frac{d}{2},
		 \, \lambda_\pm \Bigr)
\eeq
%%


==> dvb_ds_proplist_xy.tex <==
%%
Below we list the various propagators for dS$_d$.
Herein $\lambda_\pm$ is meant to carry its phase
acquired via its position in the complex plane:
%%
\begin{align}
	\lambda_\pm = \, \frac{1}{2} - \frac{1}{4}
		\biggl[  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! + \! \tau_y)
			  & - (1 \! + \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! - \! \tau_y)
			  \quad \\
		& \quad
		\mp i {\ssty \frac{\epsilon}{R\ds}} \, (\tau_x \!\! - \! \tau_y) \,  
		+ {\ssty \, \frac{\epsilon^2}{2R^2\ds} \,} \biggr]
		\notag
\end{align}
%%
Our Wightman function $G_\Delta^+$
agrees with the Wightman function which is given by
Spradlin, Strominger and Volovich in \cite{leshouches}.
%%
However our straightly forward computed
normalization constant is differs by a factor of $\sqrt{2}$
from the one they obtain by comparing the singular behaviour
of the propagator functions of deSitter and Minkowski spacetime.
%%
The reason for this disagreement is yet unknown to the author.
\\
Moreover our $i \epsilon$-prescription is slightly more precise than theirs.
%%
Spradlin, Strominger and Volovich use the complex shift
$(X^0-Y^0) \rightarrow (X^0-Y^0 - i \epsilon)$ in embedding space
for the $G^+ {\ssty (x,y)}$ propagator,
(but without giving further information about it).
%%
This is the same prescription as in equation (\ref{eq:dvb_mink_shift_01})
for Minkowski spacetime.
%% 
It works well when using the chordal distance $u$-terms
in equations (\ref{eq:dvb_ds40_5}) and (\ref{eq:dvb_ds40_5})
but does not produce meaningful results if the $XY$-terms need to be used.  
\\
Our prescription for the propagators $G^\mp {\ssty (x,y)}$
is $X^0 \rightarrow (X^0 \! \pm i {\ssty \frac{\epsilon}{2}})$
together with $Y^0 \rightarrow (Y^0 \! \mp i {\ssty \frac{\epsilon}{2}})$.
%%
This is the same as in equation (\ref{eq:dvb_mink_shift_02})
for Minkowski spacetime
and produces meaningful results for both $u$- and $XY$-terms.
%%
Our prescription agrees with the one of Spradlin, Strominger and Volovich
because for $G^+ {\ssty (x,y)}$ ours leads to
$(X^0 \! - \! Y^0) \rightarrow (X^0 \! - \! Y^0 \! - \! i \epsilon)$.
%%
\begin{align}
	G_{\! \Delta}^\pm \! {\ssty (\!x\!,y\!)}
	& = \, \frac{1}{\, 2 \beta} \: \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_\mp) 
\end{align}
%%
\begin{align}
	G_{\! \Delta}^{\sssty (\!1\!)} \! {\ssty (\!x\!,y\!)} \, 
	& = \, \frac{1}{\, \beta} \;\;\: \text{Re} \: \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_-) \\
%%
	G_{\! \Delta} \! {\ssty (\!x\!,y\!)} \, 
	& = \, \frac{1}{\, \beta} \; i \, \text{Im} \: \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_-) 
\end{align}
%%
\begin{align}
	G^{ \Delta}_{\!R} \! {\ssty (\!x\!,y\!)}
	& = \;\;\; \theta {\ssty (\!t_x\!-t_y\!)} \,
			\frac{1}{\, \beta} \, i \, \text{Im} \: \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_-) \\
	%%
	G^{ \Delta}_{\!A} \! {\ssty (\!x\!,y\!)}
	& = -\theta {\ssty (\!t_y\!-t_x\!)} \,
			\frac{1}{\, \beta} \, i \, \text{Im} \: \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_-) 
\end{align}
%%
\begin{align}
	G^{\,\Delta}_{\! F} \! {\ssty (\!x\!,y\!)} \, 
	& = \, \frac{1}{\, 2 \beta} \; \limepszero \,
				 F (\Delta_+, \Delta_-, {\ssty \frac{d}{2}}, \, \lambda_F) 
\end{align}
\\
%%
Therein $\lambda_F$ (with index F for Feynman)
is defined for the limit of small $\epsilon$ as
%%
\begin{align}
	\lambda_F \! & = \ub{\, \frac{1}{2} - \frac{1}{4} \Bigl[
			  (1 \! - \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! + \! \tau_y)
			  - (1 \! + \! \vec{\xi}_x \vec{\xi}_y) \cosh (\tau_x \!\! - \! \tau_y)
			  \Bigr] } _{\lambda}
		- \, i {\ssty \frac{\epsilon}{4R\ds}} \! 
			\mid \! \tau_x \!\! - \!\! \tau_y \!\! \mid \!
		- {\ssty \frac{\epsilon^2}{8R^2\ds} \,} 
		\notag
\end{align}
%%
so that the Feynman propagator is indeed symmetric:
$\, G_{\! F}^{\Delta} \! {\ssty (\!x\!,y\!)}
= G_{\! F}^{\Delta} \! {\ssty (\!y\!,x\!)}$.
%%
We observe that in contrast to AdS the sign of the $i \epsilon$-term
in the Feynman propagator
in dS spacetime is always positive except for $\tau_x \! = \tau_y$
as in Minkowski spacetime.
\\
For the propagators above the hypergeometric function
is defined by its convergent Taylor series
for all $\lambda$ with $\mid \! \lambda \! \mid \, < 1$.
The form of the propagators for $\mid \! \lambda \! \mid \, > 1$
can be obtained therefrom using (\ref{eq:hypergeo07}).
For $\mid \! \lambda \! \mid \, < 1$ we can use
(\ref{eq:dvb_ds57_7}).\\
%%
Likewise to Minkowski and AdS spacetime
we find that the propagators become singular
one the whole embedding space lightcone $\lambda=1$
while generating only one delta source at the coincidence point $x=y$.
\\
In appendix \ref{sec:props_ds_t} we also apply the DvB method
for static coordinates.
%%
We find perfect agreement in function and normalization
with the results of Spradlin, Strominger and Volovich in \cite{leshouches}.
%%
The only flaw of these coordinates is the non-invariance
of time ordering with respect to $t$ (see subsection \ref{sec:ds_timord_t}).


==> selbst.tex <==
%%
\pagebreak
%%
\\
%%\section*{Declaration of Personal Preparation}
%%
%Hereby I declare having prepared this diploma thesis
%independently myself without impermissible external help
%and having used only the cited sources and utilities. \\
%\\
%With the display of my diploma thesis
%in the libraries of the Humboldt University at Berlin I agree. \\
%\\ \\
%Berlin, 10$^{\text{th}} \!$ of January 2007 \qqquad Max Dohse
%%
%%
\vspace{2cm}
%%
\selectlanguage{german}
%%
\section*{Hilfsmittel}
%%
Diese Diplomarbeit wurde mit \LaTeX{} (MiKTeX 2.4) gesetzt.
%%
Die Graphiken wurden erstellt mit X-Fig 3.2, MS Paint 5.1,
Freehand 10.0 (Macromedia),
MathLab 7.3 (MathWorks Inc.)
und Mathematica 5.2 (Wolfram Research).
%%
\vspace{3cm}
%%
\section*{Selbst"andigkeitserkl"arung}
%%
Hiermit erkl\"are ich, die vorliegende Diplomarbeit
selbst\"andig sowie ohne unerlaubte fremde Hilfe verfasst
und nur die angegebenen Quellen und Hilfsmittel verwendet
zu haben.\\
\\
Mit der Auslage meiner Diplomarbeit
in den Bibliotheken der Humboldt Universit\"at zu Berlin
bin ich einverstanden. \\
\\ \\
Berlin, 10. Januar 2007 \qqqquad \quad \uad Max Dohse
\\ \\
\selectlanguage{english}
%%
%%
\vspace{5cm}
\thispagestyle{plain}
\pagebreak
%%

